Evolving Voices Based on Temporal Poisson Factorisation

The world is evolving and so is the vocabulary used to discuss topics in speech. Analysing political speech data from more than 30 years requires the use of flexible topic models to uncover the latent topics and their change in prevalence over time as well as the change in the vocabulary of the topics. We propose the temporal Poisson factorisation (TPF) model as an extension to the Poisson factorisation model to model sparse count data matrices obtained based on the bag-of-words assumption from text documents with time stamps. We discuss and empirically compare different model specifications for the time-varying latent variables consisting either of a flexible auto-regressive structure of order one or a random walk. Estimation is based on variational inference where we consider a combination of coordinate ascent updates with automatic differentiation using batching of documents. Suitable variational families are proposed to ease inference. We compare results obtained using independent univariate variational distributions for the time-varying latent variables to those obtained with a multivariate variant. We discuss in detail the results of the TPF model when analysing speeches from 18 sessions in the U.S. Senate (1981-2016).

==> supplement05_CAVI.tex <==

%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%               NEW SECTION                      %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!%%%
%\section{CAVI Updates} \label{supsec:CAVI}
\section{CAVI updates} \label{supsec:CAVI}

In this section we provide details on all CAVI updates. The updated variational parameters will be denoted by $\widehat{\bm \phi}_\bullet$, where $\bullet$ stands for parameter name and necessary indices depending on context. The only variational parameters for which no CAVI update is available are the variational parameters $\bm \phi_{hkv}^\loc$ and $\bm \phi_{hkv}^\covm$ for $\bm h_{kv}$. This is due to the inclusion of the corresponding parameters in  the Poisson rates after exponentiation.

\citet{BleiVI:2017} provide a general approach to find CAVI updates,  which we follow. In addition some of our updates are inspired by~\citet{gopalanhofmanblei2015scalableHPoisF}. In general, the most straightforward way to obtain CAVI updates is to differentiate~\eqref{supeq:ELBO_detail} with respect to the current block of variational parameters and find the optimal update by solving the system of estimating equations constructed by zeroing the gradients.

The updates for the auxiliary proportions $\phi_{dkv}^y$ can be deduced from~\eqref{supeq:reconstruction_tilde}:
\begin{equation} \label{supeq:cavi_aux_prop}
\widehat{\phi}_{dkv}^y \propto
\exp \left\{
\psi(\phi_{\theta dk}^\shp) - \log\phi_{\theta dk}^\rte
+ \phi_{hkv,t_d}^\loc
\right\}.
\end{equation}

Updates of the variational parameters for $\bm \theta$ and related auxiliary variables resemble the ones by~\citet{gopalanhofmanblei2015scalableHPoisF}:
\begin{align*}
    \widehat{\phi}_{\theta dk}^\shp &= a^\theta + \sum\limits_{v=1}^V y_{dv} \phi_{dkv}^y
	&&\text{and}& \quad
	\widehat{\phi}_{\theta dk}^\rte &= \dfrac{\phi_{\xi d}^\shp}{\phi_{\xi d}^\rte}
	+ \sum\limits_{v=1}^V \exp\left\{ \phi_{hkv,t_d}^\loc + \frac{1}{2}\phi_{hkv,t_d}^\sclsq\right\},
    \\
	\widehat{\phi}_{\xi d}^\shp &= a^{\xi} + K a^\theta 
	&&\text{and}& \quad
	\widehat{\phi}_{\xi d}^\rte &= b^{\xi} + \sum\limits_{k=1}^K \dfrac{\phi_{\theta dk}^\shp}{\phi_{\theta dk}^\rte}.
\end{align*}
Under a batching mechanism, we update only the (local) parameters for documents $d$ in the current batch. 

We continue with the updates for precision parameters $\tau_{kv}$. The variational shape parameters have a constant update that can be set from the very beginning:
$
\widehat{\phi}_{\tau kv }^\shp = a^{\tau} + \frac{T}{2}.
$
However, the variational rate parameters have to be updated with every iteration of the algorithm using~\eqref{supeq:E_quadratic_h_mu}:
\begin{equation*}
    \widehat{\phi}_{\tau kv }^\rte = b^{\tau} + \frac{1}{2} 
        \left[
            \Eq \T{\left(\bm h_{kv} - \ones \mu_{kv}\right)} \Delta_T\left(\delta_{kv}\right) \left(\bm h_{kv} - \ones \mu_{kv}\right)
        \right].
        %\left[
        %    \left(1+ \Eq \left(\delta_{kv}\right)^2\right) \sum \limits_{t=1}^{T-1}  \Eq \left(h_{kv,t} - \mu_{kv}\right)^2
        %    + \Eq \left(h_{kv,T} - \mu_{kv}\right)^2
        %    - \right. \\ \left.-   
        %    2\phi_{\delta kv }^\loc \sum\limits_{t=2}^{T} \Eq \left(h_{kv,t}^{} - \mu_{kv}\right) \left(h_{kv,t-1}^{} - \mu_{kv}\right)
        %\right],
\end{equation*}

The updates for the auto-regressive coefficients $\delta_{kv}$ are obtainable as it appears only in quadratic forms that can be combined. In particular,
\begin{align*}
\widehat{\phi}_{\delta kv }^\sclsq &= 
\dfrac{1}{
    \dfrac{1}{\left(\sigma^{\delta}\right)^2} 
    + \dfrac{\phi_{\tau kv }^\shp}{\phi_{\tau kv }^\rte}
    %\sum\limits_{t=1}^{T-1} \Eq \left(h_{kv,t} - \mu_{kv} \right)^2
    \Tr^0 \left( \Eq \left(\bm h_{kv} - \ones \mu_{kv}\right) \T{\left(\bm h_{kv} - \ones \mu_{kv}\right)} \right)
    },
\\
\widehat{\phi}_{\delta kv }^\loc &= 
    \widehat{\phi}_{\delta kv }^\sclsq
    \cdot
    \left[
        \dfrac{\mu^{\delta}}{\left(\sigma^{\delta}\right)^2} 
        + \dfrac{\phi_{\tau kv }^\shp}{\phi_{\tau kv }^\rte}
        %\sum\limits_{t=2}^T \Eq \left(h_{kv,t} - \mu_{kv} \right) \left(h_{kv,t-1} - \mu_{kv} \right)
        \Tr^1 \left( \Eq \left(\bm h_{kv} - \ones \mu_{kv}\right) \T{\left(\bm h_{kv} - \ones \mu_{kv}\right)} \right)
    \right],
\end{align*}
where analogously to Lemma~\ref{lemma:E_quadratic}
$$
\Eq \left(\bm h_{kv} - \ones \mu_{kv}\right) \T{\left(\bm h_{kv} - \ones \mu_{kv} \right)}
= 
\bm \phi_{hkv}^\covm + \left(\bm \phi_{hkv}^\loc - \ones \phi_{\mu kv}^\loc \right) \T{\left(\bm \phi_{hkv}^\loc - \ones \phi_{\mu kv}^\loc \right)} + \phi_{\mu kv}^\sclsq \ones \T{\ones}.
$$
Note that these updates would hold even if truncated normal distribution had been used for both prior and variational distribution. 
\begin{comment}
where (stripped of indices) we abbreviate
\begin{align*}
\Eq \left(h_t - \mu\right)^2 &= \phi_{h,t}^\sclsq + (\phi_{h,t}^\loc - \phi_{\mu}^\loc)^2 + \phi_{\mu}^\sclsq, 
\\
\Eq \left(h_t - \mu\right)\left(h_{t-1} - \mu\right) &= \phi_{h,t,t-1}^\covm + (\phi_{h,t}^\loc - \phi_{\mu}^\loc)(\phi_{h,t-1}^\loc - \phi_{\mu}^\loc) + \phi_{\mu}^\sclsq.
\end{align*}
\end{comment}

The updates for the auto-regressive means $\mu_{kv}$ have the following form:
\begin{align*}
\widehat{\phi}_{\mu kv }^\sclsq &= 
\dfrac{1}{
    \dfrac{1}{\left(\sigma^{\mu}\right)^2} 
    + \dfrac{\phi_{\tau kv }^\shp}{\phi_{\tau kv }^\rte}
    \; \T{\ones} \Eq \Delta_T\left(\delta_{kv}\right) \ones
    %\left[ 
        %1 + (T-1)(1 - 2\phi_{\delta kv }^\loc + \Eq \left(\delta_{kv} \right)^2)
    %\right]
    },
\\
\widehat{\phi}_{\mu kv }^\loc &= 
    \widehat{\phi}_{\mu kv }^\sclsq
    \cdot
    \left[
        \dfrac{\mu^{\mu}}{\left(\sigma^{\mu}\right)^2} 
        + \dfrac{\phi_{\tau kv }^\shp}{\phi_{\tau kv }^\rte}
        \; \T{\ones} \Eq \Delta_T\left(\delta_{kv}\right) \bm \phi_{hkv}^\loc
        %\left[
            %\left(1+\Eq \left(\delta_{kv} \right)^2 \right)\sum\limits_{t=\textcolor{red}{1}}^{\textcolor{red}{T-1}}\phi_{hkv,t}^\loc 
            %+ \phi_{hkv,T}^\loc 
            %- \phi_{\delta kv }^\loc \sum\limits_{t=2}^{T} \left(\phi_{hkv,t-1}^\loc + \phi_{hkv,t}^\loc\right)
        %\right]
    \right].
\end{align*}
